Classification of localizing subcategories along t-structures

We study the interplay between localizing subcategories in a stable $\infty$-category $\mathcal{C}$ with $t$-structure $(\mathcal{C}_{\geq 0}, \mathcal{C}_{\leq 0})$, the prestable $\infty$-category $\mathcal{C}_{\geq 0}$ and the abelian category $\mathcal{C}^{\heartsuit}$. We prove that weak localizing subcategories of $\mathcal{C}^{\heartsuit}$ are in bijection with the localizing subcategories of $\mathcal{C}$ where object-containment can be checked on the heart. This generalizes similar known correspondences for noetherian rings and bounded $t$-structures. We also prove that this restricts to a bijection between localizing subcategories of $\mathcal{C}^{\heartsuit}$, and localizing subcategories of $\mathcal{C}$ that are kernels of $t$-exact functors -- lifting Lurie's correspondence between localizing subcategories in $\mathcal{C}_{\geq 0}$ and $\mathcal{C}^{\heartsuit}$ to the stable category $\mathcal{C}$.

==> tex/05-synthetic_spectra.tex <==

\section{Synthetic spectra}

There are loads of interesting categories with $t$-structures throughout mathematics -- derived categories, quasi coherent sheaves, spectra. A new player on the block in stable homotopy theory is the category of synthetic spectra, $\SynE$, for some Adams type ring spectrum $E$. This is a compactly generated symmetric monoidal stable $\infty$-category, with a right complete $t$-structure compatible with filtered colimits. In other words, it is a $t$-stable category. The heart of this $t$-structure is the category of comodules over the Hopf algebroid $(E_*, E_*E)$, denoted $\Comod\EE$. This is a Grothendieck abelian subcategory of $\Mod_{E_*}$, that captures information about cooperations on $E$. 

We will not cover the theory of synthetic spectra in detail here, but referr the interested reader to the original source \cite{pstragowski_2022}. 

\subsection{Lubin--Tate theory}

Let $E=E_n$ be the height $n$ Lubin--Tate spectrum. This is an Adams type $\E_\infty$-algebra with coefficients $\pi_* E_n = W(\F_p)[\![v_1, v_2, \ldots, v_n^{\pm}]\!]$, with $v_i$ in degree $2$. We will denote the category of $E_n$-based synthetic spectra by $\Synn$. 

Let $I_k$ denote the Landweber ideal $(p, v_1, \ldots, v_{k-1})$. It is an invariant ideal generated by a finite regular sequence. 

\begin{definition}
    The $I_k$-power torsion comodule of a comodule $M\in \Comod\EE$ is defined as 
    \[
        T_{I_k}M = \{x\in M \mid I_k^r x = 0 \text{ for some } r\geq 0\}.
    \]
    We say that $M$ is $I_k$-power torsion if the canonical map $T_{I_k}M\to M$ is an equivalence. The full subcategory of $I_k$-power torsion comodules is denoted $\Comod\EE^{I_k-tors}$. 
\end{definition}

By \cite[5.10]{barthel-heard-valenzuela_2018} the category $\Comod\EE^{I_k-tors}$ is a Grothendieck abelian category. These categories form all the hereditary torsion theories of $\Comod\EE$, as proved by Barthel--Heard in \cite{barthel-heard_2018} using a similar classification of certain hereditary torsion theories in $\Comod_{\BP_*\BP}$ by Hovey--Strickland in \cite{hovey-strickland_2005a}. 

\begin{theorem}
    If $\T$ is a proper hereditary torsion theory of $\Comod\EE$, then there is an integer $0\leq k\leq n$ such that $\T\simeq \Comod\EE^{I_k-tors}$
\end{theorem}
\begin{proof}
    This is a combination of \cite[2.21]{barthel-heard_2018} and [REF], which implies that $v_{k+1}$-power torsion is equivalent to $I_{k}$-power torsion. 
\end{proof}

For the rest of the section we will focus on the maximal case $k=n$. We first prove a technical lemma that we will need later. 

\begin{lemma}
    The category of torsion comodules $\Comod\EE\Int$ is generated under filtered colimits by the $E_*$-homology of a finite type $n$ spectrum.  
\end{lemma}
\begin{proof}
    By \cite[2.21]{barthel-heard_2018} the hereditary torsion theory $\Comod\EE\Int$ in $\Comod\EE$ is the image of the hereditary torsion theory $\Comod_{\BP_*\BP}\Int$ in $\Comod_{\BP_*\BP}$ under the map 
    \[\Comod_{\BP_*\BP}\overset{\Phi}\to \Comod_{\BP_*\BP}/\Comod_{\BP_*\BP}^{I_{n+1}-tors}\simeq \Comod\EE\]
    By \cite[2.3]{hovey-strickland_2005a} the hereditary torsion theory $\Comod_{\BP_*\BP}\Int$ is generated by $\BP_*/I_n$, which we write $\Comod_{\BP_*\BP}\Int = \HTT(\BP_*/I_n)$. Under the map $\Phi$ the object $\BP_*/I_n$ is by \cite[5.3]{hovey-strickland_2005a} mapped to $v_n^{-1}\BP_*/I_n$. In particular the hereditary torsion $\Comod\EE\Int$ is generated by the image of $v_n^{-1}\BP_*/I_n$, which is $E_*\otimes_{\BP_*} v_n^{-1}\BP_*/I_n$. The hereditary torsion theory generated by this is equivalent to the one generated by $E_*/I_n$.

    By [REF] $\HTT(E_*/I_n)$ depends only on the radical of the ideal, hence we can, as earlier, choose a big enough number $k>0$ such that $E_*/I_n^k \cong E_*(\S/J)$ for some ideal $J$. In particular, this means that $\HTT(E_*/I_n)\simeq \HTT(E_*(\S/J))$. This spectrum is finite of type $n$, which finishes the proof. 
\end{proof}

\begin{remark}
    \label{rm:comodt-generated-by-EM}
    In particular this means that $\Comod\EE\Int$ is generated under filtered colimits by the image of the homology theory $E_*\:\Mn\to\Comod\EE\Int$. 
\end{remark}

As $\Comod\EE\Int$ is a hereditary torsion theory there is by \cref{thm:main} a $\pi$-stable subcategory $\M_n\Synn\subseteq \Synn$ with a right complete $t$-structure compatible with filtered colimits and $\Mn\Synn^\heart \simeq \Comod\EE\Int$. We suggestively denote this category as such, as it is related to the category of monochromatic spectra $\Mn$. 

\begin{theorem}
    \label{thm:mono-iff-syn-mono}
    If $X$ is an $E_n$-local spectrum, then $\nu X \in \Mn\Synn$ if and only if $X\in \M_n$. 
\end{theorem}
\begin{proof}
    Assume that $\nu X$ lies in the $\pi$-stable localizing subcategory $\Mn\Synn$. Then we know that $\pi_k^\heart \nu X \in \Comod\EE\Int$ for all $k$. By \cite[4.21]{pstragowski_2022} there are equivalences $\pi_k^\heart \nu X\cong E_* X[-k]$, and we have by \cite{aambo_2024} that $X\in \Mn$ if and only if $E_* X\in \Comod\EE\Int$, which is enough as it is closed under shifts.  

    Similarily, if $X\in \Mn$ then $E_*X\cong \pi_*^\heart \nu X\in \Comod\EE\Int$, hence $\nu X\in \Mn\Synn$ as it it a $\pi$-stable localizing subcategory. 
\end{proof}

In light of the above result we call $\Mn\Synn$ the category of \emph{monochromatic} ($E$-based) \emph{synthetic spectra}. 




\begin{remark}
    By \cite[4.23]{pstragowski_2022} we can lift the fiber sequence $\S\overset{p}\to\S\to\S/p$ to a fiber sequence $\nu \S \overset{\widetilde{p}}\to \nu \S\to \nu (\S/p)$ in synthetic spectra $\SynE$ as it induces a short exact sequence 
    \[0\to E_* \overset{\cdot p}\to E_*\to E_*/p\to 0\]
    on $E_*$-homology. In particular, $\nu (\S/p)\simeq (\nu \S)/\widetilde{p}$. Similar ideas were used by Burklund to prove the existence of $\E_1$ structures on Moore spectra in \cite{burklund_2022}. 
    
    Now, as $\nu (\S/p)$ is a finite number of cones away from the sphere, it is a compact object in $\SynE$. We can iterate this construction to lift generalized Moore spectra into the synthetic setting. These are then compact synthetic objects that behave similarily to finite type $n$ spectra. 
\end{remark}

\begin{lemma}
    There is a finite type $n$ spectrum $F$ whose synthetic analog is compact. 
\end{lemma}
\begin{proof}
    Let $I_n$ be the Landweber ideal $(p,v_1, v_2, \ldots, v_{n-1})$. By (an $E$-local version of) \cite[4.14]{hovey-strickland_99} there is a finite type $n$ generalized Moore spectrum $\S_n/J$ for $J=(p^{i_0}, v_1^{i_1}, \ldots, v_{n-1}^{i_{n-1}})$ constructed by iterated fiber sequences. These fiber sequences all induce short exact sequences on $E_*$-homology, hence we can lift them to fiber sequences in synthetic $\Synn$ by \cite[4.23]{pstragowski_2022}. In particular we have $\nu (\S_n/J) \simeq (\nu \S_n)/\widetilde{J}$ for $\widetilde{J} = (\widetilde{p}^{i_0}, \widetilde{v}_1^{i_1}, \ldots, \widetilde{v}_{n-1}^{i_{n-1}})$. Since we used a finite number of shifts and fiber sequences, $\nu \S_n/J$ is a compact object in $\Synn$. 
\end{proof}

\begin{definition}
    A synthetic type $n$ spectrum $\nu F$ is a compact synthetic spectrum that is the synthetic analog of a finite type $n$ spectrum. 
\end{definition} 

\begin{theorem}
    \label{thm:MnSynn-generated-by-vF}
    Any synthetic type $n$ spectrum $\nu F$ generates $\Mn\Synn$ under filtered colimits.  
\end{theorem}
\begin{proof}
    As $\nu$ is a colimit preserving functor we know that $\nu(\Loc(F))\subseteq \Loc(\nu F)$. Any finite type $n$ spectrum generates $\Mn$ under filtered colimits, hence $\Loc(F) \simeq \Mn$. In particular, $\Loc(\nu F)$ contains the synthetic analog $\nu M$ of any monochromatic spectrum $M\in \Mn$. 

    Now, let $X$ be a synthetic spectrum in $\Mn\Synn$ that is not in the localizing subcategory $\Loc(\nu F)$. 
    
    
    In particular this means that there are no equivalences $X\to \colim_\alpha \nu M_\alpha$ to a filtered colimit of synthetic analogs of monochromatic spectra $M_\alpha$, for any choice of $M_\alpha$. As the $t$-structure on $\Mn\Synn$ is right complete and compatible with filtered colimits, the heart-valued homotopy groups functors $\pi_k^\heart$ are jointly conservative and commutes with filtered colimits. In particular, any map $X\to \colim_\alpha \nu M_\alpha$ as above does not induce an equivalence $\pi_k^\heart X \to \pi_k^\heart \colim_\alpha \nu M_\alpha$ for any $k$ and any choice of filtered colimit. 

    By the properties of $\pi_k^\heart$ mentioned we have
    \begin{align*}
        \pi_k^\heart \colim_\alpha \nu M_\alpha 
        &\simeq \colim_\alpha \pi_k^\heart \nu M_\alpha \\
        &\simeq \colim_\alpha E_*M_\alpha[-k].
    \end{align*}
    But the collection of comodules $E_*M$ for all $M\in \Mn$ generates $\Comod\EE\Int$ under filtered colimits by \cref{rm:comodt-generated-by-EM}, hence the comodules $\pi_k^\heart \nu X$ cannot lie in the hereditary torsion theory $\Comod\EE\Int$, which contradicts the $\pi$-stability of $\Mn\Synn$. Hence no such synthetic spectrum can exist.
\end{proof}

\begin{remark}
    \label{rm:MnSynn-generated-by-vMs}
    In particular this means that the collection of synthetic analogs of monochromatic spectra $\{\nu M\}$ for all $M\in \Mn$ generates $\Mn\Synn$ under filtered colimits. This further implies that $\Mn\Synn$ is a full stable subcategory of the category of hypercomplete synthetic spectra, as any $P\in \Mn$ is also $E_n$-local, and the collection of synthetic spectra $\nu X$ for $X\in \Spn$ generates $\Synn$ under filtered colimits. 
\end{remark}

%%%%%%%%% Previous stuff, does not work I think. 
    
    % Let $X\in \Mn\Synn$. Since $\Synn$ is generated under filtered colimits by the image of $\nu\colon \SpE\to \Synn$ we have a presentation $X\simeq \colim_\alpha \nu P_\alpha$ for $P_\alpha\in \SpE$. Applying $\tau^{-1}$ we get 
    % \begin{align*}
    %     \tau^{-1}X
    %     &\simeq \tau^{-1}\colim_\alpha \nu P_\alpha \\
    %     &\simeq \colim_\alpha \tau^{-1}\nu P_\alpha \\
    %     &\simeq \colim_\alpha P_\alpha.
    % \end{align*}
    % As $X$ was in $\Mn\Synn$ we know that $\tau^{-1}X\in \Mn$, hence also the colimit $\colim_\alpha P_\alpha \in \Mn$. As monochromatization $M_n\colon \SpE\to \Mn$ is a smashing colocalization we then have 
    % \begin{align*}
    %     \tau^{-1}X 
    %     &\simeq M_n \tau^{-1}X \\
    %     &\simeq M_n \colim_\alpha P_\alpha \\
    %     &\simeq \colim_\alpha M_n P_\alpha.
    % \end{align*}
    % Hence we have a map 
    % \[\colim_\alpha \nu P_\alpha \to \colim_\alpha \nu M_n P\]
    % and we want to show that this is an equivalence. 



    % First, note that the collection of $\nu P$'s generates the (non-hypercomplete) category of $E=E_n$-based synthetic spectra $\SynE$ by \cite[4.14]{pstragowski_2022}. The synthetic spectrum $\nu P$ is by \cite[5.4, 5.5]{pstragowski_2022} hypercomplete if and only if $P$ is $E$-local. Hence, the hypercomplete category is -- as it is closed under colimits -- generated by the collection of $\nu P$'s for $E$-local finite projective spectra $P$. 

    % Now, if any one of these generators $\nu P$ lie in $\Mn\Synn$, then $P$ is by \cref{thm:mono-iff-syn-mono} a monochromatic spectrum, i.e. $\P\in \Mn$. Since $\Mn\Synn$ is closed under colimits this implies that any $X\in \Mn\Synn$ is a filtered colimit of finite projectives $\nu P$ such that $P\in \Mn$. By \cite{aambo_2024} this happens precicely when $E_*P \in \Comod\EE\Int$. 

\begin{lemma}
    \label{lm:MnSynn-localizing-ideal}
    The localizing subcategory $\Mn\Synn\subseteq \SynE$ is a localizing ideal. 
\end{lemma}
\begin{proof}
    We need to show that for any $X\in \Mn\Synn$ and $Y\in \Synn$, that $X\otimes Y\in \Mn\Synn$. By the fact that $\Mn\Synn$ is closed under filtered colimits, $\otimes$ commutes with filtered colimits separately in each variable, and we have explicit descriptions of the generators in both $\Synn$ and $\Mn\Synn$, we can reduce to the case $X = \nu M$ for some $M\in \Mn$ and $Y=\nu P$ for some $E$-local finite projective $P \in \Spn$. 
    
    We have $\nu M \otimes \nu P \simeq \nu(M\otimes P)$ by \cite[4.24]{pstragowski_2022}. Hence, by \cref{thm:mono-iff-syn-mono} we know that $\nu(M\otimes P)\in \Mn\Synn$ if and only if $M\otimes P \in \Mn$, which holds as $\Mn$ is a localizing ideal of $\Spn$.
\end{proof}

\begin{construction}
    It follows from \cref{lm:MnSynn-localizing-ideal} that $\Mn\Synn$ inherits a symmetric monoidal structure from $\SynE$, making it a compactly generated symmetric monoidal stable $\infty$-category. In the language of \cite{barthel-heard-valenzuela_2018} $(\SynE, \nu F)$ is a local duality context for any choice of synthetic type $n$ spectrum $\nu F$. Hence there is a right adjoint $\Gamma_n$ to the fully faithful inclusion $\Mn\Synn\hookrightarrow \SynE$, which by \cite[2.21]{barthel-heard-valenzuela_2018} is a smashing colocalization. In particular, it preserves all colimits. 
\end{construction}

\begin{remark}
    By local duality there is a dual category $L_{\nu F}\SynE$ equivalent to $\Mn\Synn$. In upcoming work with Marius Nielsen we claim that such a category is a good model for studying $K(n)$-local synthetic phenomena, and prove some properties for this category.  
\end{remark}

\begin{proposition}
    The colocalization map $M_n X\to X$ of spectra, induces a synthetic colocalization map $\nu M_n X\to \nu X$ such that $\Gamma_n \nu X \simeq \nu M_n X$. 
\end{proposition}
\begin{proof}
    There is a natural map $\nu M_n X \to \Gamma_n \nu X$ given as the composite 
    \[\nu M_n X\overset{\simeq}\longleftarrow \Gamma_n \nu M_n X \to \Gamma_n \nu X,\]
    where the first map is an equivalence due to $\Gamma_n$ being a colocalization and $\nu M_n X \in \Mn\SynE$ by \cref{thm:mono-iff-syn-mono}. 
\end{proof}
















As synthetic spectra acts as a one parameter deformation of stable homotopy theory, one can wonder wether $\Mn\Synn$ inherits deformation-like properties, and if that is the case, what does it deform between? Fortunately, the answer is yes to the former, and the answer to the latter is the natural answer.

\begin{theorem}
    \label{thm:Mn-generic-fiber}
    The symmetric monoidal equivalence $\Synn[\tau^{-1}]\simeq \Spn$ induces a symmetric monoidal equivalence $\Mn\Synn[\tau^{-1}]\simeq \Mn$. In other words, the generic fiber of the deformation is $\Mn$. 
\end{theorem}
\begin{proof}
    There is a Barr--Beck adjunction 
    \[
        \begin{tikzcd}
            \Synn \arrow[r, "\tau^{-1}", yshift=2pt] & \Spn \arrow[l, "Y", yshift=-2pt]
        \end{tikzcd}
    \]
    exhibiting the equivalence $\Synn[\tau^{-1}]\simeq \Spn$. Here $Y$ is the spectral Yoneda embedding. This means, in particular, that $\Spn \simeq \Mod_{\tau^{-1}\S_n^{0,0}}(\Synn)$. By \cite[A.6]{aambo_2024} this induces a Barr--beck adjunction on localizing subcategories
    \[
        \begin{tikzcd}
            \Mn\Synn \simeq \Loc^\otimes(\nu F) \arrow[r, "\tau^{-1}", yshift=2pt] & \Loc^\otimes(F)\simeq \Mn \arrow[l, "\bar{Y}", yshift=-2pt]
        \end{tikzcd}
    \]
    where the first equivalence is due to \cref{thm:MnSynn-generated-by-vF} and \cref{lm:MnSynn-localizing-ideal}. Here the left adjoint is the restriction of $\tau^{-1}$ to $\Mn\Synn$ and the right adjoint $\bar{Y}$ is the composition $\Gamma_n \circ Y$. 
\end{proof}










\begin{theorem}
    \label{thm:Mn-special-fiber}
\end{theorem}

















\subsection{Brown--Peterson homology}

For this section we let $E = \BP$, the Brown--Peterson spectrum. It is an Adams type ring spectrum with coefficients $\Z_{(p)}[v_1, v_2, \ldots]$, where $v_i$ lies in degree $2p^i-2$. 

\begin{theorem}[{\cite[B, C]{hovey-strickland_2005a}}]
    Let $\T$ be a hereditary torsion theory in $\Comod_{\BP_*\BP}$ containing a non-trivial compact comodule. Then there is an integer $k\geq -1$ such that $\T\simeq \Comod_{\BP_*\BP}^{I_k-tors}$. 
\end{theorem}

==> tex/09-testing.tex <==

Questions:

Can the equivalence between Grothendieck prestable categories and stable categories with a nice t-structure be realized by an equivalence of (∞,2)-functors? In particular Sp(-) and (-)^{>=0} 











% Before we start with the localizing subcategories, let us add a technical result that we will need for some of the below theory to work properly. 

% \begin{theorem}
%     The category of hypercomplete $E_n$-based synthetic spectra is closed under filtered colimits and tensoring with objects $X\in \SynE$. 
% \end{theorem}
% \begin{proof}
%     By \cite{clausen-mathew_2021} this is equivalent $\1^h \otimes X$ being hypercomplete for any $X\in \SynE$, where $\1^h$ denotes the hypercompletion of the unit. The unit in $\SynE$ is the synthetic analog of the sphere, $\nu \S$, and it's hypercompletion is by \cite{pstragowski_2022} the synthetic analog of the $E_n$-local sphere, $\1^h \simeq \nu \S_n$. Since $\SynE$ is generated under filtered colimits by $\nu P$'s, for $P$ finite projective, and $\otimes$ commutes with filtered colimits, we can reduce to the case $X=\nu P$. 
% \end{proof}
